DeepMetis: Augmenting a Deep Learning Test Set to Increase its Mutation Score

Deep Learning (DL) components are routinely integrated into software systems that need to perform complex tasks such as image or natural language processing. The adequacy of the test data used to test such systems can be assessed by their ability to expose artificially injected faults (mutations) that simulate real DL faults. In this paper, we describe an approach to automatically generate new test inputs that can be used to augment the existing test set so that its capability to detect DL mutations increases. Our tool DeepMetis implements a search based input generation strategy. To account for the non-determinism of the training and the mutation processes, our fitness function involves multiple instances of the DL model under test. Experimental results show that \tool is effective at augmenting the given test set, increasing its capability to detect mutants by 63% on average. A leave-one-out experiment shows that the augmented test set is capable of exposing unseen mutants, which simulate the occurrence of yet undetected faults.

==> model.tex <==
\section{Model-based Input Representation}
\label{model}


In the empirical evaluation of this work, we consider both a classification problem and a regression problem. The classification problem is handwritten digit recognition, while the regression one is eye gaze prediction. Since our input generation technique is model-based, we need a model of handwritten digits and a model of the eye to be manipulated during automated input generation. We describe them in this section.

\subsection{Handwritten Digit Recognition} 
Our source of handwritten digit samples is the MNIST database~\cite{LecunBBH98}. Its inputs are originally encoded as $28\times28$  images, with greyscale levels that range from 0 to 255. We model them as combinations of B\'ezier curves by adopting Scalable Vector Graphics (SVG)\footnote{\url{https://www.w3.org/Graphics/SVG/}} as their representation. SVG is an XML-based vector image format for two-dimensional graphics that can represent shapes as the combination of cubic and quadratic B\'ezier curves. %Figure~\ref{fig:svg_model} shows an MNIST image paired with its SVG model and its description. 
The control parameters that determine the shape of the modelled digit are the start point, the end point and the control points \textit{c1} and \textit{c2} that define each B\'ezier segment.

This representation ensures that the smoothness and curvature of handwritten shapes is preserved and that images remain realistic even after (minor) manipulation of the B\'ezier curve parameters~\cite{RiccioFSE20}. We use the Potrace algorithm~\cite{Selinger03} to transform an original input image into its SVG model representation. This algorithm performs a sequence of operations, including binarisation, despeckling and smoothing, to obtain a smooth vector image starting from a bitmap. 


%\begin{figure}
%\centering
%  \includegraphics[width=0.8\linewidth]{figures/SVGmodel.png}
%  \caption{(1) An input in the format accepted by the image classifier, (2) the corresponding vector image, (3) its model representation returned by Potrace \vincenzo{This image is the same in DeepJanus, I can change it a little bit}}
%  \label{fig:svg_model}
%\end{figure}

To transform an SVG model into a $28\times28$  grayscale image, we perform a rasterisation operation by means of the functionalities offered by two popular open source graphic libraries (i.e. LibRsvg\footnote{\url{https://wiki.gnome.org/Projects/LibRsvg}} and Cairo\footnote{\url{https://www.cairographics.org}}).


\subsection{Gaze Prediction} \label{sec:gazemodel}

\begin{figure}
\centering
  \includegraphics[width=0.8\linewidth]{figures/unity_model.png}
  \caption{Unity Model \nargiz{the image is now taken from the reference paper that was used to build the model and is used as an example, if we want such an image and have space for it, I will quickly produce a similar one.}}
  \label{fig:unity_model}
\end{figure}

Eye gaze prediction is becoming increasingly important in several domains, such as assisted car driving, where monitoring the driver's attention is a key safety condition, and the recent advances of deep learning have made the task achievable with high accuracy.
In particular, we focus on image-based gaze estimation, which directly uses images of eyes as input to predict the gaze direction.
Our case study is based on a multimodal convolutional neural network (CNN) available in a public GitHub repository~\cite{unityEyesModel}, which provides an implementation based on the LeNet network architecture~\cite{lecun:1998} following the approach described in~\cite{zhang:2015}. The CNN learns the mapping from eye image and \textit{2D} head angle (\textit{yaw} and \textit{pitch}) to \textit{2D} eye gaze angle (\textit{polar} and \textit{azimuthal} angles \paolo{@Nargiz: please, double check}). The dataset that we used for training and testing is supplied along with the model and consists of 129,285 eye region images synthesised with \textit{UnityEyes} --- a freely available rendering framework~\cite{wood:2016}. Each image is accompanied by a \textit{JSON} file describing \textit{2D} head angle and \textit{2D} eye angle, as well as other parameters used to generate the image, such as skin texture and various lighting features. When presented to a model for training and prediction,  images are converted to grayscale and cropped to $60\times36$ pixels. The head angle and eye angle, which represent the second input to the model and the ground truth, respectively, are converted into radians. An example of an input image along with the model architecture can be found on Figure \ref{fig:unity_model}. 

Our model of the eye consists of all the parameters used by UnityEyes to generate an eye image. Such parameters are recorded by UnityEyes in a JSON file. They can be divided into two groups: those that cover various aspects related to the eye appearance  (head angle, eye angle, pupil size, iris size, iris texture, skin texture) and others that describe the lighting (texture, rotation, ambient intensity,  exposure, for image-based lighting, and rotation and intensity, for directional lighting). It is important to notice that only some of these parameters are directly controllable when asking UnityEyes to generate new images, namely head angle and eye angle. The others are decided internally by UnityEyes and are just reported as a JSON file that accompanies the generated image. For each controllable input, consisting of the head and eye angles, it is possible to request UnityEyes to generate an arbitrary number of eye images, differing among each other by the other, not directly controllable, parameters.

When manipulating UnityEye's parameters for the purpose of test input generation, we need to know the range in which each parameter falls in order to ensure the validity of the new values. 
%While head and eye angles can be specified by a user of the framework prior to the beginning of the generation process, all other parameters cannot be explicitly controlled by the user and their values are selected and decided by the framework during the generation. 
Thus, for head and eye angles, we use the ranges suggested in the \textit{UnityEyes} interface. To learn the valid ranges for the remaining parameters, we have generated a dataset of more than 1 million images and analysed the generated \textit{JSON} files. The identified ranges and the script used for such analysis are available in our replication package~\cite{replicationPkg}.

Once we have mutated the parameters of the eye model, the next step would be to obtain an input image that corresponds to the new values. Since only a small subset of parameters can be controlled by a user of the framework, to find the desired solution, we generate a high number of images and \textit{JSON} file pairs ($\sim$200) \nargiz{number can change if we decide so} under the same controllable parameters, and then we search for the pair which is closest to the target parameter list, which includes the uncontrollable parameters.



